Rethinking Targeted Adversarial Attacks For Neural Machine Translation

Targeted adversarial attacks are widely used to evaluate the robustness of neural machine translation systems. Unfortunately, this paper first identifies a critical issue in the existing settings of NMT targeted adversarial attacks, where their attacking results are largely overestimated. To this end, this paper presents a new setting for NMT targeted adversarial attacks that could lead to reliable attacking results. Under the new setting, it then proposes a Targeted Word Gradient adversarial Attack (TWGA) method to craft adversarial examples. Experimental results demonstrate that our proposed setting could provide faithful attacking results for targeted adversarial attacks on NMT systems, and the proposed TWGA method can effectively attack such victim NMT systems. In-depth analyses on a large-scale dataset further illustrate some valuable findings. 1 Our code and data are available at https://github.com/wujunjie1998/TWGA.

==> sections/related_work.tex <==
\section{Related Work}
\label{related work}

%\paragraph{Targeted Adversarial Attacks in NLP.}

%\paragraph{Adversarial Attacks on NMT Systems.} 
%A proper strategy for evaluating the adversarial robustness of NMT systems is crucial for enhancing the stability of such systems. 
Although achieving great translation performances, current NMT systems are unstable when facing adversarial attacks. Existing adversarial attacks for NMT systems mainly belong to two categories: crafting adversarial examples to analyze the performance degradation of NMT models in terms of sentence-level metrics ~\cite{michel2019evaluation,zou2019reinforced,niu2020evaluating,zhang2021crafting,wan2022paeg,lai2022generating}; or measuring translation errors on targeted words against word-level attacks~\cite{ebrahimi2018adversarial, wallace2020imitation, cheng2020seq2sick}. 
While most works in this field lie in the former category, the latter category is gaining more research interests 
and their problem settings are summarized in \sref{previous settings}. %can be summarized as: making a pre-defined targeted word to be included in the translation output~\cite{cheng2020seq2sick} or excluding a targeted word from the current translation output~\cite{ebrahimi2018adversarial,wallace2020imitation}.
However, as demonstrated by \sref{revisiting}, attacking results obtained from both settings are largely overestimated. 
In contrast, our proposed attack setting addresses this issue by constraining the tokens that can be perturbed when crafting adversarial examples and thus can provide more reliable attacking results. 

%Besides, %targeted adversarial attacks have also been used to investigate linguistic phenomena in NMT. 
%\citet{emelin2020detecting} apply a targeted attack %targeting ambiguous words 
%to detect word sense disambiguation biases in NMT, yet targeted words in their setting are limited to homographs-polysemous nouns. In contrast, our proposed setting aims to investigate translation errors on more types of general words, which helps to obtain crucial findings from broader perspectives.
%evaluation framework targets the translation of named entities. Since the meanings of named entities are usually crucial and unambiguous within different contexts, they are very suitable for providing more reliable adversarial robustness evaluation results. 

%\noindent \textbf{Named Entity Translation.} \quad How to correctly translate named entities has always been an important research question for decades~\cite{knight1997machine,al2002named,yang2009chinese}. More recently, with the rapid growth of NMT models, various methods have been proposed to fuse external named entity-related knowledge into both the pre-training~\cite{hu2021deep} and the regular training~\cite{ugawa2018neural,torregrosa2020aspects} stages of NMT systems to improve their named entity translation quality. Yet, to the best of our knowledge, no efforts have been made on evaluating the adversarial robustness of NMT systems by targeting named entity translation. 



